Neutrino Imaging of the Galactic Centre and Millisecond Pulsar Population

In this work, we consider the possible presence of a large population of millisecond pulsars in the Galactic Centre. Their direct detection would be challenging due to severe pulse broadening caused by scattering of radiation. We propose a new method to constrain their population with neutrino imaging of the Galactic Centre. Millisecond pulsars are proposed cosmic-ray accelerators. The high-energy protons they produce will collide with the baryonic matter in the central molecular zone to create charged and neutral pions that decay into neutrinos and $\gamma$-rays, respectively. The specific neutrino and $\gamma$-ray fluxes must be below their corresponding observed values, allowing us to put a conservative upper limit on the millisecond pulsar population of N_MSP < 10,000 within a galacto-centric radius of 20 pc. This upper limit is sensitive to the proton acceleration efficiency of the pulsars, but is less dependent on the particle injection spectral index and the choice of mass tracers. The population will be better constrained when high resolution neutrino observations of the Galactic Centre become available. The presence of these millisecond pulsars can account for the $\gamma$-ray excess in the Galactic Centre.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

